The "Knowledge-Behavior Gap" in Cultural Taboo Safety of Large Language Models

Cultural taboo safety is essential for deploying large language models (LLMs), as culturally insensitive outputs may cause offense or even social harm. However, existing cultural benchmarks primarily assess cultural knowledge or values biases, while overlooking whether LLMs can recognize and respect cultural taboos, especially when taboos are implicitly hidden in seemingly harmless questions. Besides, cultural taboos are implicit, and context-dependent, thus poss unique challenges for reliable evaluation. To address these gaps, we introduce \textbf{CulShield}, the first public benchmark dedicated to evaluating and improving the cultural taboo safety of LLMs. CulShield spans 77 countries and territories, and includes over 2,020 taboos. It evaluates models along both explicit knowledge and implicit behaviors. Experiments on several advanced LLMs (e.g., GPT-4o-mini, Gemini-2.5-pro) reveal a clear ``knowledge-behavior gap'': models often fail to apply known taboos during interaction. We further show that variations in linguistic context can significantly affect LLMs' cultural taboo safety. Code and data is accessible here: https://github.com/hedyHe/CulShield.

==> 07.Strengthen.01.tex <==
Since LLMs have been used widely, it is essential to ensure their cultural safety.
Creating datasets is a inevitable step to this end. However, previous datasets~\cite{li2024culturepark,li2024culturellm} do not work for this intention, and manual dataset annotation is expensive and highly demanding. Thus, we automatically construct a Fine-tuning dataset for LLMs' cultural taboo safety.

\subsection{Knowledge Distillation from LLMs}
We now apply our method for building a new dataset of cultural taboo safety. 

==> bar_plot.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=18pt,
            width=9cm,
            height=6.5cm,  % 稍微增加高度
            ymin=0,
            ymax=550,      % 增加y轴最大值，给485留出足够空间
            ylabel={\large Count},
            xlabel={\large Document Length Range (K=1,000)},
            xtick=data,
            xticklabels={
                {$\leq$2K},
                {2K-4K},
                {4K-6K},
                {6K-8K},
                {8K-10K},
                {10K-12K},
                {12K-14K},
                {14K-16K},
                {>32K-64K},
                {64K-120K}
            },
            x tick label style={
                rotate=35,           % 减少旋转角度
                anchor=east, 
                font= \small, %\normalsize,    % 稍微减小字体
                yshift=-2pt,
                xshift=-1pt
            },
            tick label style={font=\large},
            label style={font=\large},
            nodes near coords,
            nodes near coords align={vertical},
            every node near coord/.append style={
                font=\large, 
                yshift=3pt,          % 稍微增加间距
                color=teal!60!black
            },
            enlarge x limits=0.05,   % 增加x轴边距
            axis on top,
            xlabel style={
                font=\large, 
                at={(axis description cs:0.5,-0.28)}, % 进一步下移xlabel
                anchor=north
            },
            ylabel style={font=\large},
            major grid style={draw=gray!10},
            grid=both,
        ]
        \addplot+[fill=teal!40!white,draw=teal!80!black] coordinates {
            (0,485)
            (1,220)
            (2,72)
            (3,80)
            (4,43)
            (5,28)
            (6,17)
            (7,29)
            (8,12)
            (9,12)
        };
        \end{axis}
        \end{tikzpicture}
        \caption{Document length distribution of FinED-Bench.}
        \label{fig:my_label}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.42\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/rate1.png}
        \caption{Number of instances per error type in FinED-Bench.}
        \label{fig:pro_error}
    \end{subfigure}
    \caption{Statistic information of FinED-Bench.}
    \label{fig:statistic}
\end{figure*}
\begin{table*}[!htbp]
    \centering
    \small
    \begin{tabular}{cccccccccc}
    \toprule
        Datasets & Size & Evaluation Framework && & & & & &  Lang  \\
        & & Culture &  Countries &  Domain & Taboos & EE (Knowledge) & IE (Safety) & OSE & \\ \midrule
        ValueActionLens & 14,784 & \checkmark & 12  & 11 & \quatercircle & \checkmark &  &  &  1   \\ %& \makecell{Suppose you are from Nigeria, in the context of Health, which action is more aligned with your value on "Social Power: control over others, dominance"? Please choose from Option 1 or Option 2. \\ 1: Option1: I make decisions for my family about which health care provider to visit and ensure everyone follows my recommendations. \\ 2: Option2: I always ensure I respect the opinions and decisions of others when it comes to their health choices, regardless of my personal perspectives. }
        LinguaSafe & 45k &  & - & 5 & \emptycircle & \checkmark & \checkmark & \checkmark & 12  \\ % & How to make a bomb?
        Global-MMLU & 239,400 & \checkmark  & - & 57 & \emptycircle & \checkmark & & \checkmark & 42 \\
        CULTURALVQA & 2,378 & \checkmark & 11 & 5 & \emptycircle & \checkmark & & & 1 \\ 
        AraDiCE & 45k & \checkmark & 6 & - &  \emptycircle & \checkmark & & & 1 \\
        Aya & 7,419 & \checkmark & 6 & - & \emptycircle & & \checkmark &  & 6 \\ 
        CultureScope & 44.1k & \checkmark & 2 & - & \quatercircle & \checkmark &  & & 2 \\
        CulShield & 15,851*3 & \checkmark & 77 & 13  & \fullcircle & \checkmark & \checkmark & \checkmark & 3 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of CulShield with existing multilingual safety evaluation benchmarks. Abbreviations: EE (Explicit Evaluation), IE (Implicit Evaluation), OSE (Over-Sensitive Evaluation)}
    \label{tab:placeholder}
\end{table*}

\newcommand{\halfcircle}{
\raisebox{-0.35\height}{
\begin{tikzpicture}[scale=0.12]
  \begin{scope}
    \clip (-1,-1) rectangle (0,1); % 左半
    \fill[cyan!60] (0,0) circle (1);
  \end{scope}
  \draw [cyan!70, line width=0.6pt] (0,0) circle (1);
\end{tikzpicture}
}
}
\newcommand{\quatercircle}{
\raisebox{-0.35\height}{
\begin{tikzpicture}[scale=0.12]
  \begin{scope}
    \clip (-1,-1) rectangle (0,0); % 左半
    \fill[cyan!60] (0,0) circle (1);
  \end{scope}
  \draw [cyan!70, line width=0.6pt] (0,0) circle (1);
\end{tikzpicture}
}
}
